ucTrace: A Multi-Layer Profiling Tool for UCX-driven Communication

UCX is a communication framework that enables low-latency, high-bandwidth communication in HPC systems. With its unified API, UCX facilitates efficient data transfers across multi-node CPU-GPU clusters. UCX is widely used as the transport layer for MPI, particularly in GPU-aware implementations. However, existing profiling tools lack fine-grained communication traces at the UCX level, do not capture transport-layer behavior, or are limited to specific MPI implementations. To address these gaps, we introduce ucTrace, a novel profiler that exposes and visualizes UCX-driven communication in HPC environments. ucTrace provides insights into MPI workflows by profiling message passing at the UCX level, linking operations between hosts and devices (e.g., GPUs and NICs) directly to their originating MPI functions. Through interactive visualizations of process- and device-specific interactions, ucTrace helps system administrators, library and application developers optimize performance and debug communication patterns in large-scale workloads. We demonstrate ucTrace's features through a wide range of experiments including MPI point-to-point behavior under different UCX settings, Allreduce comparisons across MPI libraries, communication analysis of a linear solver, NUMA binding effects, and profiling of GROMACS MD simulations with GPU acceleration at scale. ucTrace is publicly available at https://github.com/ParCoreLab/ucTrace.

==> docs.tex <==
Google doc for discussions
https://docs.google.com/document/d/1THPbHoymnXlTgZAfoD9aMlcu1Jv23Mx7659YVlKd7h4/edit?tab=t.0#heading=h.qfncvve1hept

==> tables/hardware.tex <==
% Matrix reordering survey
%
% date: 2023-03-06
%
% authors:
%
%  James D. Trotter <james@simula.no>
%
% Hardware

\begin{table*}
  \centering
  \caption{Hardware used in our experiments.}
  %\linespread{0.85}
  %\renewcommand{\arraystretch}{1.2}
  %\setlength{\tabcolsep}{3pt}
  %\footnotesize
  \small\sffamily
  \begin{tabularx}{\textwidth}{
      >{\hsize=1.2\hsize\raggedright\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
%      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.7\hsize\raggedleft\arraybackslash}X
      >{\hsize=0.8\hsize\raggedleft\arraybackslash}X}
    \toprule
    & {\small Skylake}
    & {\small Ice Lake}
%    & {\small Xeon-C}
    & {\small Naples}
    & {\small Rome}
    & {\small Milan A}
    & {\small Milan B}
    & {\small TX2}
    & {\small Hi1620} \\

%    \midrule

%    partition
%    & {\footnotesize\ttfamily{}xeongold16q}
%    & {\footnotesize\ttfamily{}habanaq}
%    & {\footnotesize\ttfamily{}dgx2q}
%    & {\footnotesize\ttfamily{}defq}
%    & {\footnotesize\ttfamily{}rome16q}
%    & {\footnotesize\ttfamily{}fpgaq}
%    & {\footnotesize\ttfamily{}milanq}
%    & {\footnotesize\ttfamily{}armq}
%    & {\footnotesize\ttfamily{}huaq} \\

    \midrule

    CPUs
    & Intel Xeon Gold 6130
    & Intel Xeon Platinum 8360Y
%    & Intel Xeon Platinum 8168
    & AMD Epyc 7601
    & AMD Epyc 7302P
    & AMD Epyc 7413
    & AMD Epyc 7763
    & Cavium TX2 CN9980
    & HiSilicon Kunpeng 920-6426 \\ \addlinespace


    Instr. set
    & x86-64
    & x86-64
%    & x86-64
    & x86-64
    & x86-64
    & x86-64
    & x86-64
    & ARMv8.1
    & ARMv8.2 \\

    Microarch.
    & Skylake
    & Ice Lake
%    & Skylake
    & Zen
    & Zen 2
    & Zen 3
    & Zen 3
    & Vulcan
    & TaiShan v110 \\

    Sockets
    & 2
    & 2
%    & 2
    & 2
    & 1
    & 2
    & 2
    & 2
    & 2 \\

    Cores
    & $2\times 16$
    & $2\times 36$
%    & $2\times 24$
    & $2\times 32$
    & $1\times 16$
    & $2\times 24$
    & $2\times 64$
    & $2\times 32$
    & $2\times 64$ \\

    Freq.~[GHz]
    & $1.9$--$3.6$
    & $2.4$--$3.5$
%    & $2.5$--$3.7$
    & $2.7$--$3.2$
    & $1.5$--$3.3$
    & $2.5$--$3.5$
    & $2.5$--$3.5$
    & $2.0$--$2.5$
    & $2.6$ \\

    L1I/core [KiB]
    & 32
    & 32
%    & 32
    & 64
    & 32
    & 32
    & 32
    & 32
    & 64 \\

    L1D/core [KiB]
    & 32
    & 48
%    & 32
    & 32
    & 32
    & 32
    & 32
    & 32
    & 64 \\

    L2/core [KiB]
    & 1024
    & 1280
%    & 1024
    & 512
    & 512
    & 512
    & 512
    & 256
    & 512 \\

    L3/socket [MiB]
    & 22
    & 54
%    & 33
    & 64
    & 16
    & 128
    & 256
    & 32
    & 64 \\

%    Mem. channels
%    & $2\times 6$
%    & $2\times 8$
%%    & $2\times 6$
%    & $2\times 8$
%    & $1\times 8$
%    & $2\times 8$
%    & $2\times 8$
%    & $2\times 8$
%    & $2\times 8$ \\

    Bandwidth~[GB/s]
    & 256
    & 409.6
%    & 256
    & 342
    & 204.8
    & 409.6
    & 409.6
    & 342
    & 342 \\

%    Triad [GB/s]
%    & 147.1
%    & 294.5
%%    & 137.4
%    & 169.7
%    & 90.9
%    & 206.8
%    & 256.5
%    & 236.4
%    & 260.4 \\

    % fp64 flops/core/cycle
    % & $32$
    % & $32$
    % & $ 8$
    % & $16$
    % & $16$
    % & $16$
    % & $ 8$
    % & $ 4$ \\

    % Theoretical fp64 perf.
    % & $1\,946$\,Gflop/s
    % & $3\,840$\,Gflop/s
    % & $1\,382$\,Gflop/s
    % &    $768$\,Gflop/s
    % & $5\,120$\,Gflop/s ?
    % & $5\,120$\,Gflop/s
    % & $1\,024$\,Gflop/s
    % & $1\,331$\,Gflop/s \\

    \bottomrule
  \end{tabularx}
  \label{tab:hardware}
\end{table*}

